The Immersion of Directed Multi-graphs in Embedding Fields. Generalisations

The purpose of this paper is to outline a generalised model for representing hybrids of relational-categorical, symbolic, perceptual-sensory and perceptual-latent data, so as to embody, in the same architectural data layer, representations for the input, output and latent tensors. This variety of representation is currently used by various machine-learning models in computer vision, NLP/NLU, reinforcement learning which allows for direct application of cross-domain queries and functions. This is achieved by endowing a directed Tensor-Typed Multi-Graph with at least some edge attributes which represent the embeddings from various latent spaces, so as to define, construct and compute new similarity and distance relationships between and across tensorial forms, including visual, linguistic, auditory latent representations, thus stitching the logical-categorical view of the observed universe to the Bayesian/statistical view.

==> 04_Article_WordCount.tex <==
\section*{Word Counts}
This section is \textit{not} included in the word count.



\subsection*{Notes on JPhysD article}
\begin{itemize}
    \item Abstract: 150 words, unreferenced
    % \item Sections: Introduction Results, Discussion, Online Methods. Topical subheadings allowed in Results and Online Methods
    \item Main text: short format 4500 words, long is 8500 words.
    \item No limit in number of figures
    % \item References: Up to 40
\end{itemize}

\section*{Statistics on word count}

\immediate\write18{texcount -utf8 -nobib -merge -sum -dir 01_Article_MainText.tex > \jobname.wcdetail }
\verbatiminput{\jobname.wcdetail}


==> 05_ToDoList.tex <==
\section*{Paper to do list:}

\begin{todolist}
    % \item[\done] Play with LEGO
    % \item[\done] Acknowledgements
    % \item[\done] Author contributions
    % \item[\done] Handle how Dix paper is introduced
    % \item[\done] Move Event detection dataset to main text (?)
    % \item Check video links
    % \item Check link and completeness of software/hardware availability
    % \item Check list of references
    % \item Complete Materials and methods
    % \item[\done] Add Christophe's reference to the bibliography
    % \item consider merging main text and methods bibliography(?)
    % \item[\done] Decide whether to include the dual color imaging with CD4/actin or not
    % \item[\done] Tidy up SuppInfo
    % \item dSTORM to STORM in SuppInfo + Movies
    
    \item[\done] Write abstract (RFL, RH)
    \item Obtain data for figures and design figures (KT)
    
    

\end{todolist}



